GPTDrawer: Enhancing Visual Synthesis through ChatGPT

In the burgeoning field of AI-driven image generation, the quest for precision and relevance in response to textual prompts remains paramount. This paper introduces GPTDrawer, an innovative pipeline that leverages the generative prowess of GPT-based models to enhance the visual synthesis process. Our methodology employs a novel algorithm that iteratively refines input prompts using keyword extraction, semantic analysis, and image-text congruence evaluation. By integrating ChatGPT for natural language processing and Stable Diffusion for image generation, GPTDrawer produces a batch of images that undergo successive refinement cycles, guided by cosine similarity metrics until a threshold of semantic alignment is attained. The results demonstrate a marked improvement in the fidelity of images generated in accordance with user-defined prompts, showcasing the system's ability to interpret and visualize complex semantic constructs. The implications of this work extend to various applications, from creative arts to design automation, setting a new benchmark for AI-assisted creative processes.

==> sec/0_abstract.tex <==
\begin{abstract}
    Large Artificial Intelligence
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}

Stable Diffusion (SD), as delineated by Rombach et al. \cite{rombach2021highresolution}, represents a paradigm shift in the domain of latent diffusion models. It's premised on the ability to transmute text-based prompts into high-resolution visual constructs. These prompts act not just as triggers but as foundational descriptors delineating the contours of the visual content the model generates.

However, preliminary investigations have highlighted a potential limitation in the SD model. As the complexity and granularity of textual descriptions escalate, the model occasionally manifests a decrement in its efficacy, failing to produce visualizations that congruently mirror the descriptive intricacies of the provided text.

Simultaneously, there's been a surge in advancements in the domain of natural language processing, epitomized by models such as ChatGPT. Its prowess in comprehending, interpreting, and generating refined text offers a tantalizing proposition: Can ChatGPT be harnessed as an auxiliary tool, a "prompt architect", to enhance the congruence between intricate textual prompts and the visual outputs of the Stable Diffusion model?

In the ensuing discourse, this paper seeks to elucidate the potential of amalgamating ChatGPT's linguistic capabilities with the visual generation potential of SD. By employing ChatGPT as an intermediary, the objective is to optimize the textual prompts to be more receptive to SD's processing dynamics. Section 3 provides a meticulous examination of empirical examples, shedding light on the viability and efficacy of this integrative approach.

\section{Methodology}

\input{utils/algorithm}

\input{utils/framework}

\subsection{Overview}
\label{sec:overview}
In the proposed workflow delineated in Algorithm~\ref{algorithm:pipeline} and Figure~\ref{fig/framework}, the system commences by ingesting an input prompt, denoted as \textit{P}. This input is subject to a rigorous extraction procedure executed by the language model, \textit{ChatGPT}, which distills an array of keywords, symbolized as $\mathbf{w}$. These keywords serve as the cornerstone for the \textit{Stable Diffusion} algorithm, which synthesizes a batch of preliminary visual representations, designated as $I_{B}$.

Each visual output within the batch $I_{B}$ is subsequently encoded through an Image Encoder, expressed as $E_{image}(I_{B})$. Concurrently, the keyword array $\mathbf{w}$ undergoes a similar encoding process to yield $E_{text}(\mathbf{w})$. The crux of the process involves computing a cosine similarity measure, $Sim_{cos}$, to quantify the alignment between the encoded representations of the visual outputs and the keywords.

The iterative refinement cycle is triggered if the similarity metric for any keyword fails to surpass a pre-established threshold, $T$. During this phase, \textit{ChatGPT} is tasked with refining both the prompt \textit{P} and the individual keywords $\mathbf{w}_{i}$. This refinement is informed by the discrepancies identified through the similarity assessment. After prompt adjustment, the \textit{Stable Diffusion} model generates a new set of images, $I_{B}^{'}$, which are then re-assessed for conformity to the refined keywords.

This recursive process is iterated until the similarity for all keywords meets or exceeds the threshold, at which point the process concludes. The culmination of this methodology is the generation of a set of refined images $I_B$, each associated with a maximal cosine similarity measure, $Sim_{cos}$. The outputs are thus ensured to be in close adherence to the semantic intent encapsulated within the original input prompt.


\subsection{Input Prompt Reception}

This is the entry point of the process, where the user provides the system with an initial prompt. The system initializes by awaiting an input from the user.
Once received, the input undergoes preliminary validation to check for readability and structural integrity.

\subsection{Keyword Extraction}

At this stage, the primary objective is to distill the most essential terms from the input.
The system uses natural language processing techniques to identify and segment key terms.
Algorithms like TF-IDF (Term Frequency-Inverse Document Frequency) might be employed to prioritize terms based on their prominence in the input.
Stop words and other irrelevant terms are filtered out to maintain the purity of the extracted keywords.


\subsection{BLIP Model Evaluation}

The BLIP model is pivotal, acting as the decision-making entity that discerns the relevance of extracted keywords.
Keywords are presented to the BLIP model in a sequential or batched manner.
The model, trained on vast amounts of data, assesses the contextual importance of each keyword.
Through deep learning techniques, the model predicts the TRUE or FALSE label for each keyword based on its relevance to the desired context.

\subsection{Keyword Filtering}

This step is about actioning the insights gleaned from the BLIP model's evaluation.
Keywords with a TRUE label are segregated and stored in a primary array, earmarked for the final refined prompt.
Keywords with a FALSE label are either discarded or stored separately for potential future analysis or feedback loops.
This filtering ensures that only the most pertinent terms make their way to the refined prompt.

\subsection{Prompt Refinement}

The culmination of the process, this stage is where the refined prompt is crafted.
The system intelligently stitches together the TRUE labeled keywords, maintaining a logical and coherent structure.
Grammatical and syntactical adjustments are made to ensure that the refined prompt is not only accurate but also easily comprehensible.
This prompt is a more focused version of the original, aiming to yield better results in subsequent tasks.

\subsection{Output}

The end result of the entire methodology is presented to the user.
The refined prompt is displayed to the user via the chosen interface.
Alongside this, feedback mechanisms might be incorporated to gather user insights on the efficacy of the refinement, aiding in future iterations of the system.

\section{Experiments}
For example, we want to use the Stable Diffusion model to generate a graph in CyberPunk style with the following description: 

``The neon lights flickered and reflected off the rain-slicked streets as the protagonist made their way through the bustling crowds of the futuristic city. The air was thick with the hum of technology and the scent of fried food from the street vendors. Hovering cars zoomed overhead, casting shadows on the towering skyscrapers that loomed above. The sound of a distant explosion echoed through the alleyways, a reminder of the constant danger that lurked in this high-tech metropolis."

The Stable diffusion model generates Fig.~\ref{Fig.main1}., which doesn't completely fit the description of our CyberPunk Scene.

However, if we use ChatGPT as a prompt engineer, let it summarize the description given above, it gives ``neon lights, rain-slicked streets, protagonist, futuristic city, hum of technology, scent of fried food, street vendors, hovering cars, shadows, towering skyscrapers, distant explosion, alleyways, constant danger, high-tech metropolis." It gives Fig.~\ref{Fig.main2}., which fits the description and CyberPunk style very well.

\vspace{-.1in}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{figs/grid1.png}
    \caption{Figure Generated by SD Directly} 
    \label{Fig.main1}
\end{figure}



\vspace{-.2in}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{figs/grid2.png}
    \caption{Figure Generated by SD with ChatGPT as a prompt engineer} 
    \label{Fig.main2}
\end{figure}

==> utils/table_result.tex <==
%\vspace{-.2in}
\begin{table}[h]
\centering
\begin{tabular}{cc}
  \includegraphics[width=0.45\linewidth]{figs/scene1_baseline.png} & 
  \includegraphics[width=0.45\linewidth]{figs/scene1_GPT.png} \\
  Baseline & GPTDrawer \\
\end{tabular}
\caption{Generation results for Scene I}
\label{tab:images_1}
\end{table}

